The Mixed Aggregate Preference Logit Model: A Machine Learning Approach to Modeling Unobserved Heterogeneity in Discrete Choice Analysis

This paper introduces the Mixed Aggregate Preference Logit (MAPL, pronounced "maple'') model, a novel class of discrete choice models that leverages machine learning to model unobserved heterogeneity in discrete choice analysis. The traditional mixed logit model (also known as "random parameters logit'') parameterizes preference heterogeneity through assumptions about feature-specific heterogeneity distributions. These parameters are also typically assumed to be linearly added in a random utility (or random regret) model. MAPL models relax these assumptions by instead directly relating model inputs to parameters of alternative-specific distributions of aggregate preference heterogeneity, with no feature-level assumptions required. MAPL models eliminate the need to make any assumption about the functional form of the latent decision model, freeing modelers from potential misspecification errors. In a simulation experiment, we demonstrate that a single MAPL model specification is capable of correctly modeling multiple different data-generating processes with different forms of utility and heterogeneity specifications. MAPL models advance machine-learning-based choice models by accounting for unobserved heterogeneity. Further, MAPL models can be leveraged by traditional choice modelers as a diagnostic tool for identifying utility and heterogeneity misspecification.

==> Archive/HAVAN-Paper/Tikz/diagram.tex <==
\begin{tikzpicture}
        \draw[white](0,0)--(0,0);
        \begin{scope}[shift={(0,0)}]
        
            \draw[->] (-1.5,0) -- (1.5,0) node[right] {};
            
        
            % Adjusted standard deviation
            \def\stddev{0.35}
        
            % Normal distribution curve
            \draw[smooth, thick, domain=-1:1] plot (\x, {exp(-\x*\x/(2*\stddev*\stddev))/(sqrt(2*pi)*\stddev)});
        
            
    
        \end{scope}

    
        
        \node[black] at (1.75,1) {=};
        
        \node[black] at (4.75,1) {\Huge $\cdot$};
        \node[black] at (5.75,1) {\large $x_{ijt}$};
        \node[black] at (6.75,1) {+};
        \node[black] at (9.25,1) {\Huge $\cdot$};
        \node[black] at (10.25,1) {\large $z_{ijt}$};
        \node[black, align=center] at (8,-.45) {$z$-related\\preference};
        \node[black, align=center] at (3.5,-.45) {$x$-related\\preference};
        
        \node[black, align=center] at (0,-.45) {Heterogeneous\\preferences};
        \begin{scope}[shift={(8,0)}]
        
            \draw[->] (-1.5,0) -- (1.5,0) node[right] {};
            
        
            % Adjusted standard deviation
            \def\stddev{0.25}
        
            % Normal distribution curve
            \draw[smooth, thick, domain=-1:1] plot (\x, {exp(-\x*\x/(2*\stddev*\stddev))/(sqrt(2*pi)*\stddev)});
        
            
    
        \end{scope}

        \begin{scope}[shift={(3.5,0)}]
        
            \draw[->] (-1.5,0) -- (1.5,0) node[right] {};
            
        
            % Adjusted standard deviation
            \def\stddev{0.2}
        
            % Normal distribution curve
            \draw[smooth, thick, domain=-1:1] plot (\x, {exp(-\x*\x/(2*\stddev*\stddev))/(sqrt(2*pi)*\stddev)});
        
            
    
        \end{scope}

        \draw[red, <->, thick] (3.75, 2.1) .. controls (4.4,3) and (6.875,3) .. (7.25, 2.1);
        \node[red, align=center] at (5.75,3.5) {\large Mixed logit models estimate\\ \large constituent mixing distribution parameters};
        \draw[blue, ->, thick] (5.75, .65) .. controls (5.5,-2) and (5,-2) .. (1, -1);
        \draw[blue, -, thick] (10.25, .65) .. controls (10,-2) and (9.5,-2) .. (4, -1.62);
        \node[blue, align=center] at (5.75,-3) {\large HAVAN Framework directly relates model inputs\\ \large to distributional parameters of aggregate observables-related preference};
    \end{tikzpicture}

==> Archive/HAVAN-Paper/scratch.tex <==
The central computational bottleneck to mixed logit estimation is the integration by simulation process necessary to estimate mixed logit models. Recent work has shown that the required number of simulated draws required (i.e. compute and memory resources) to yield appropriate estimates of model log-likelihood is both relatively large and scales with the number of mixing distributions being estimated \citep[Table 5]{Czajkowski2019}.


Primarily, the proposed framework seeks to 1) expand flexibility of discrete choice model specification, 2) reduce the computational burden of model estimation, and 3) allow for a variety of decision-making paradigms such as utility maximization, regret minimization, or otherwise.


independent mixing distributions \cite{Forsythe2023,Helveston2015, Philip2021, Guo2021,Kavalec1999}, convenient mixing distributions \cite{Forsythe2023,Helveston2015,Philip2021,Revelt1998, Guo2021,Kavalec1999}, or consumer homogeneity for a subset of product attributes \citep{Philip2021, Guo2021, Kavalec1999} ---.

Relaxing some of these assumptions through various non/semi-parametric distributional representation of mixing distribution has been the focus of much recent work \citep{Fosgerau2013,Train2016, Krueger2020}. However, relaxations of distributional form can increase the computational burden of model estimation \citep[Table 1]{Krueger2020} - a burden that can be quite large even when assuming convenient distributional forms \citep{Arteaga2022}. Although the works referenced thus far generally rely on models of consumer utility, mixed logit models can also be leveraged in models of consumer regret \citep[p.79]{Chorus2012}. In sum, the theoretical promises of mixed logit models cannot be implemented due to practical issues regarding modern mixed logit specification and estimation. In this paper, we propose a new framework for discrete choice model specification and estimation that will make the hitherto impractical theoretical promises of the mixed logit practical. 

==> scratch.tex <==
The central computational bottleneck to mixed logit estimation is the integration by simulation process necessary to estimate mixed logit models. Recent work has shown that the required number of simulated draws required (i.e. compute and memory resources) to yield appropriate estimates of model log-likelihood is both relatively large and scales with the number of mixing distributions being estimated \citep[Table 5]{Czajkowski2019}.


Primarily, the proposed framework seeks to 1) expand flexibility of discrete choice model specification, 2) reduce the computational burden of model estimation, and 3) allow for a variety of decision-making paradigms such as utility maximization, regret minimization, or otherwise.


independent mixing distributions \cite{Forsythe2023,Helveston2015, Philip2021, Guo2021,Kavalec1999}, convenient mixing distributions \cite{Forsythe2023,Helveston2015,Philip2021,Revelt1998, Guo2021,Kavalec1999}, or consumer homogeneity for a subset of product attributes \citep{Philip2021, Guo2021, Kavalec1999} ---.

Relaxing some of these assumptions through various non/semi-parametric distributional representation of mixing distribution has been the focus of much recent work \citep{Fosgerau2013,Train2016, Krueger2020}. However, relaxations of distributional form can increase the computational burden of model estimation \citep[Table 1]{Krueger2020} - a burden that can be quite large even when assuming convenient distributional forms \citep{Arteaga2022}. Although the works referenced thus far generally rely on models of consumer utility, mixed logit models can also be leveraged in models of consumer regret \citep[p.79]{Chorus2012}. In sum, the theoretical promises of mixed logit models cannot be implemented due to practical issues regarding modern mixed logit specification and estimation. In this paper, we propose a new framework for discrete choice model specification and estimation that will make the hitherto impractical theoretical promises of the mixed logit practical. 
